Rethinking Backdoor Attacks

In a backdoor attack, an adversary inserts maliciously constructed backdoor examples into a training set to make the resulting model vulnerable to manipulation. Defending against such attacks typically involves viewing these inserted examples as outliers in the training set and using techniques from robust statistics to detect and remove them. In this work, we present a different approach to the backdoor attack problem. Specifically, we show that without structural information about the training data distribution, backdoor attacks are indistinguishable from naturally-occurring features in the data--and thus impossible to "detect" in a general sense. Then, guided by this observation, we revisit existing defenses against backdoor attacks and characterize the (often latent) assumptions they make and on which they depend. Finally, we explore an alternative perspective on backdoor attacks: one that assumes these attacks correspond to the strongest feature in the training data. Under this assumption (which we make formal) we develop a new primitive for detecting backdoor attacks. Our primitive naturally gives rise to a detection algorithm that comes with theoretical guarantees and is effective in practice.

==> editor.tex <==
\usepackage[normalem]{ulem}
\usepackage{xcolor}

\newcommand{\ai}[1]{{\color{blue} [AI: #1]}}

\newcommand{\add}[1]{{\color{blue!70!black} #1}}
\newcommand{\del}[1]{{\color{red!50} \sout{#1}}}
\newcommand{\rep}[2]{{\color{red!50} \sout{#1}}{\color{blue!70!black} #2}}
\newcommand{\cmt}[2]{{\color{red!15!blue!65} #1}\footnote{{\color{red!60!black} $\leftarrow$ #2}}}
\newcommand{\gram}[1]{{\color{red!70!gray} {\bfseries #1}}}
\newcommand{\hlt}[1]{\gram{#1}}

\newcommand{\scrcmd}{\textsuperscript}
\newcommand{\scr}[1]{\scrcmd{#1}}
\newcommand{\myst}{{\hypersetup{hidelinks}\bf \color{purple} \hyperref[exp:myst]{\scr{mysterious}}}}
\newcommand{\cit}{{\hypersetup{hidelinks}\bf \color{green!50!black} \hyperref[exp:cit]{\scr{cite}}}}
\newcommand{\wdy}{{\hypersetup{hidelinks}\bf \color{orange} \hyperref[exp:wdy]{\scr{wordy}}}}
\newcommand{\unimp}{{\hypersetup{hidelinks}\bf \color{blue!70} \hyperref[exp:unimp]{\scr{unimportant}}}}
\newcommand{\awk}{{\hypersetup{hidelinks}\bf \color{red} \hyperref[exp:awk]{\scr{awkward}}}}

\newcommand{\ExplanationPage}{
\newpage
\onecolumn

\section*{Explanation of editor markings}
\renewcommand{\scrcmd}{}
\hypersetup{hidelinks}
\begin{itemize}
\item \label{exp:myst} \myst: This will probably come across as mysterious to readers who don't already have the context to know what you're talking about.
\item \label{exp:cit} \cit: You should try to cite something here (e.g. to give an example of, or justification for, what you just talked about).
\item \label{exp:wdy} \wdy: This is stated in more words than is necessary and can probably be shortened.
\item \label{exp:unimp} \unimp: This is not that important relative to the length/prominence it's currently given.
\item \label{exp:awk} \awk: Awkward grammar (overly complex and/or not clear what a given subclause/modifier corresponds to).
\end{itemize}
}
